Facilitating Parallel Fuzzing with mutually-exclusive Task Distribution

Fuzz testing, or fuzzing, has become one of the de facto standard techniques for bug finding in the software industry. In general, fuzzing provides various inputs to the target program to discover unhandled exceptions and crashes. In business sectors where the time budget is limited, software vendors often launch many fuzzing instances in parallel as common means of increasing code coverage. However, most of the popular fuzzing tools in their parallel mode-naively run multiple instances concurrently, without elaborate distribution of workload. This can lead different instances to explore overlapped code regions, eventually reducing the benefits of concurrency. In this paper, we propose a general model to describe parallel fuzzing. This model distributes mutually-exclusive but similarly-weighted tasks to different instances, facilitating concurrency and also fairness across instances. Following this model, we develop a solution, called AFL-EDGE, to improve the parallel mode of AFL, considering a round of mutations to a unique seed as a task and adopting edge coverage to define the uniqueness of a seed. We have implemented AFL-EDGE on top of AFL and evaluated the implementation with AFL on 9 widely used benchmark programs. It shows that AFL-EDGE can benefit the edge coverage of AFL. In a 24-hour test, the increase of edge coverage brought by AFL-EDGE to AFL ranges from 9.49% to 10.20%, depending on the number of instances. As a side benefit, we discovered 14 previously unknown bugs.

==> appendices.tex <==
\appendix



%\section{Existing Algorithms of Seed Distillation}
%\label{app:distillalg}
%In our evaluation, we compare Algorithm~\ref{alg:taskdistribute} with three %existing seed distillation algorithms, \emph{Unweighted}, \emph{Weight-Time}, and \emph{Weight-Size}. We describe the three algorithms as follows.

%In this paper, we consider three existing distillation algorithms in parallel with ours : unweighted greedy algorithm from \cite{Abdelnur2010Spectral} (notated as \emph{Unweighted}), a minimal set cover with weight of execution time algorithm (notated as \emph{Weight-Time}) and a minimal set cover weighted by size algorithm from AFL-CMIN \cite{aflaflcm94:online}(notated as \emph{Weight-Size}). The first algorithm and last algorithm have been proposed in the previous literature and online document. We realized and evaluated these three algorithms in experiment and the result is shown in Table~ \ref{tab:seedistill}. \\
%All above algorithms take a corpus with size ${n}$ as input, the output is the reduced corpus with size ${k}$, where ${k}$ $<$ ${n}$. All the results from these three algorithms can ensure that the coverage from reduced corpus equals to the original corpus coverage. It should be noted that there are other seed distillation algorithms, such as Hot Set and Random Set introduced in \cite{seedoptimize}. However, we do not included them in our evaluation since these distillation algorithms cause coverage lost after size reduction. \\ %$\bigcup{}=\bigcup_{i=1}^{n} \vec{E}_{i}$\;



%Corresponding to the coverage-based evaluation metric, this algorithm always picks the seed with maximal edge number on current the set of uncovered edges to obtain full coverage eventually. This algorithm is easy to implement but without guarantee of the smallest corpus size as output. Its specifics follow Algorithm~\ref{alg:unweighted}.  \\ 

%\begin{algorithm}
%\SetAlgoLined
%\Input{Family ${F}$ of set ${S_1}$ ... ${S_{n}}$ ; uncovered\_edges}
%\Output{The Minimized family ${R}$}
% \While{uncovered\_edges \neq $\emptyset$}{
%  ${S_{max}}$ ${=}$ seed in ${F}$ which has largest number of uncovered edges %\;
%  add ${S_{max}}$ to ${R}$ \;
%  remove ${S_{max}}$ hit edges from uncovered\_edges \;
%  remove ${S_{max}}$ from ${F}$
%  }
%  return ${R}$
%\caption{Unweighted Algorithm.\label{alg:unweighted}}
%\end{algorithm}





%Considering the time consumption and resources to flip the bits, fuzzing always prefers many smaller seeds with diversity rather than single input with large size. Weighting by file size makes algorithm always picks the seed with smallest size. Moreover, AFL-CMIN takes edge counts as a metrics to enhance the weighted size algorithm and its specifics follow Algorithm~\ref{alg:size-weighted}. AFL-CMIN is a widely used tool in practice and its experiment result is the one most close to our algorithm. 

%The intuition of this algorithm, which was introduced by \cite{woo2013black-box}, is that there will be much more fuzz runs if we ultimately run the fastest seeds. This algorithm always picks the seed with shortest execution time and its specifics follow Algorithm~\ref{alg:time-weighted}. For lack of consideration of other critical metrics, it is not very effective on size reducing.\\


%\begin{algorithm}
%\SetAlgoLined
%\Input{Family ${F}$ of Set ${S_1}$ ... ${S_{n}}$ ; uncovered\_edges ; Execution %time of each seed ${T_{s}}$ }
%\Output{The Minimized family ${R}$}
% \While{uncovered\_edges $\neq$ $\emptyset$}{
%  ${S_{T_{min}}}$ ${=}$ seed in F which has the shortest execution time \;
%   add ${S_{T_{min}}}$ to ${R}$ \;
%   remove ${S_{T_{min}}}$ hit edges from uncovered\_edges \;
%   remove ${S_{T_{min}}}$ from ${F}$ \;
% }
% return ${R}$
% \caption{Weight-Time Algorithm.\label{alg:time-weighted}}
%\end{algorithm}

%\noindent\textbf{Size-Weighted (AFL-CMIN)} 
%Considering the time consumption and resources to flip the bits, fuzzing always prefers many smaller seeds with diversity rather than single input with large size. Weighting by file size makes algorithm always picks the seed with smallest size. Moreover, AFL-CMIN takes edge counts as a metrics to enhance the weighted size algorithm and its specifics follow Algorithm~\ref{alg:size-weighted}. AFL-CMIN is a widely used tool in practice and its experiment result is the one most close to our algorithm. 

%\begin{algorithm}
%\SetAlgoLined
%\Input{Family ${F}$ of Set ${S_1}$ ... ${S_{n}}$ ; uncovered\_edges ; hit count %of each edge ${E_{hit}}$ }
%\Output{The Minimized family ${R}$}
% \While{uncovered\_edges $\neq$ $\emptyset$}{
%    target\_edge = max(${E_{hit}}$);\\
 %   ${S_{S_{max}}}$ ${=}$ seed in ${F}$ which covers target\_edge meanwhile covers largest number of uncovered\_edges; \\
%    add ${S_{S_{max}}}$ to ${R}$;\\
%    remove ${S_{S_{max}}}$ hit edges from uncovered\_edges;\\
%    remove ${S_{S_{max}}}$ from ${F}$;\\
    

% }
% return ${R}$
% \caption{Weight-Size Algorithm.\label{alg:size-weighted}}
%\end{algorithm}


%\section{Increase of Edge Coverage across 24 Hours}
%In Fig.~\ref{fig:codecov}, we present the results of edge coverage with our 9 %benchmark programs across 24 hours.
\clearpage
\input{tab/code-cov}
\clearpage

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip , keepaspectratio]{headshot/Yifan Wang.jpg}}]{Yifan Wang}
is a Ph.D. student in the Department of Computer Science at Stevens Institute of Technology. She received her M.S. in Computer Science from New York Institute of Technology in 2017. Her recent research focus is on software security.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip, keepaspectratio]{headshot/Yuchen Zhang.jpg}}]{Yuchen Zhang}
obtained his BA in Computer Science at Boston University, and took master courses in Brandeis University. He is currently in his second year of his Ph.D. in Computer Science at Stevens Institute of Technology. His research interests center around Software, System Security, and malware.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip, keepaspectratio]{headshot/Chenbin Pang.jpg}}]{Chengbin Pang}
received the B.E. degree in Computer Science and Technology from Shandong University in 2017. He is currently pursuing the Ph.D. degree in the Department of Computer Science and Technology, Nanjing University. His current research interests include system and software security.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip, keepaspectratio]{headshot/peng_li.jpeg}}]{Peng Li} is a security engineer at ByteDance. He received his Ph.D. degree from school of computing in University of Utah.  His research interests include scalable static analysis, practical fuzzing, and hybrid testing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip, keepaspectratio]{headshot/Triandopoulos_Photo.jpeg}}]{Nikolaos Triandopoulos} is an Associate Professor in the Department of Computer Science of Stevens Institute of Technology. His research interests broadly span security, privacy and cryptography. From 2010 to 2016, he was a Principal Research Scientist at RSA Labs, carrying out research on cloud security, identity management and enterprise security. Prior to RSA Labs, he held research faculty positions at Boston University and Brown University.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip, keepaspectratio]{headshot/Jun Xu.jpg}}]{Jun Xu}
 is an Assistant Professor in the Department of Computer Science at Stevens Institute of Technology. He received his Ph.D. from the College of Information Sciences and Technology at the Pennsylvania State University. His research area covers software security, system security, and malware.

\end{IEEEbiography}

% \begin{IEEEbiographynophoto}{Yifan Wang}
% Biography text here.
% \end{IEEEbiographynophoto}

==> tab/afl-stat.tex <==
\begin{table*}[t!]
\scriptsize
\caption{Statistical results of our evaluation with \afl in 24 hours. In the table, ``\textsf{overlap reduction rate}'' means the average percentage of seeds that the corresponding solution cuts from each instance; ``\textsf{edge coverage increase}'' stands for the increase of code coverage that the corresponding solution brings to \afl; \textsf{p-value} demonstrates the statistical significance of the increase of code coverage (the smaller, the better); and ``\textsf{coverage overlap rate}'' shows how much of the code covered by \afl is also covered by the corresponding solution.}
\label{tab:afl:stat}
\vspace{0.5em}
\begin{tabular}{p{0.85cm}|wl{1.0cm}||p{0.70cm}p{0.70cm}p{0.80cm}|p{0.74cm}p{0.74cm}p{0.74cm}|p{1.1cm}p{1.1cm}p{1.2cm}|p{0.85cm}p{0.85cm}p{0.70cm}}
\toprule[0.5pt]
\toprule[0.5pt]
\multirow{2} {*}{\textbf{\normalsize{Prog.}}} & 
\multirow{2} {*}{\textbf{\normalsize{Setting}}} &
\multicolumn{12}{c}{\textbf{\large{Statistical evaluation results with 2, 4, and 8 instances (\afl).}}} \\ \cline{3-14}
& & \multicolumn{3}{c|}{\textsf{overlap reduction rate}} & \multicolumn{3}{c|}{\textsf{edge coverage increase}} & \multicolumn{3}{c|}{\textsf{p-value}} & \multicolumn{3}{c}{\textsf{coverage overlap rate}} \\

\hline
\multirow{3}{*}{\sc objdump} &{\sc pafl}  &60.55 & 80.77 & 89.49            &1.93 &0.01  & 0.30                 &0.321    &0.715    &0.102      &95.46 &94.87 &95.81
\\
& {\sc p-fuzz}  &46.72 &53.47 &62.54            &5.08 & 2.26 & 3.02                & 0.072   & 0.032   & ${2.91*e^{-4}}$      &96.82 &96.27 &97.89 \\

& {\sc afl-edge} & 63.74 & 63.20 & 62.37             &7.63 & 7.31 & 3.06         & 0.001 & 0.038 & 0.025                       &97.54 & 98.34 & 98.53 \\




\hline

\multirow{3}{*}{\sc readelf} &{\sc pafl}        &81.23 &86.81 &88.41          &5.56 &-3.24 &-3.58        &0.033  &0.189  &0.117      & 92.54 &92.13 &92.87                                      \\

&{\sc p-fuzz}        &46.75 & 43.75 & 45.37          &7.17 &3.77 &6.01        &0.040  &0.006  &${3.92*e^{-5}}$                &98.85 &98.51 &97.96                                     \\

&{\sc afl-edge}  &45.92 & 43.75 & 42.47          &12.15 &6.96 &8.43        &0.050  &0.020  & 0.001       &97.52 &97.21 &97.69                                     \\


\hline

\multirow{3}{*}{\sc tiff2pdf} &{\sc pafl}  &64.07 &79.72 &81.24           &3.44 &0.38 &4.95           &0.004 &0.049 &0.293      &96.96 &91.28 &93.81                                      \\

&{\sc p-fuzz}       &42.18 & 60.12 & 64.13          &5.50 &6.27 &8.48          &0.007 &0.040 &0.042               &98.51 &97.06 &97.91                                     \\

&{\sc afl-edge}    &62.38& 59.47& 58.54          &9.01& 5.63& 11.19        &${7.69*e^{-5}}$&0.021&${2.96*e^{-4}}$       &98.49& 95.98& 99.14                   \\




\hline
\multirow{3}{*}{\sc nm-new} &{\sc pafl}    &46.18 &52.56 &55.90                         &4.04 &4.76  &0.20             &0.098  &0.072  & 0.187                &96.64 &96.18  &97.53                                       \\

&{\sc p-fuzz}    &43.62& 55.63& 60.21                        &4.52& 7.08& 3.81           & 0.001 &0.032 &0.002               &97.63& 98.14& 98.12                                     \\

 &{\sc afl-edge}      &59.87& 58.46& 60.12                        &6.78  &6.61 &3.59         &0.027 &0.076 &0.001               &96.25& 96.85& 98.53        \\

\hline

\multirow{3}{*}{\sc nasm} &{\sc pafl}        &64.17 &82.65  &54.70          &5.51 &14.58  &2.37             &0.050   &0.012  &0.057               &99.78 &99.25  &99.78                               \\

&{\sc p-fuzz}        &10.01& 10.95& 8.21        &8.93& 9.18& 8.05           & ${2.46*e^{-6}}$ &${2.32*e^{-5}}$ &${3.64*e^{-6}}$              &98.96& 98.33& 94.25                              \\

&{\sc afl-edge}    &67.88& 68.25& 66.84                        &13.85& 22.59& 7.61           & ${1.73*e^{-8}}$ & ${1.85*e^{-7}}$ &${1.43*e^{-4}}$              &99.24& 99.26& 99.26            \\



\hline

\multirow{3}{*}{\sc tiff2ps} &{\sc pafl}  &57.08 & 81.93 & 89.21       &7.81  &14.99  &8.66   &0.034 & 0.019 &0.024  &82.25 & 89.85& 96.56  \\

&{\sc p-fuzz}  &44.00& 60.69& 66.42       &7.50 & 12.32 & 9.54   &${8.24*e^{-4}}$&${5.74*e^{-8}}$&${6.63*e^{-4}}$  &97.05 & 97.45 & 98.02  \\

&{\sc afl-edge}  &53.36 &58.46  &52.82  &10.43& 13.52 & 7.29           & ${1.66*e^{-5}}$ &${5.01*e^{-5}}$ &${5.88*e^{-4}}$    & 96.98 & 96.50& 97.15          \\


\hline
\multirow{3}{*}{\sc tcpdump} &{\sc pafl}        &66.36 &80.32 &84.37        & 8.20 &10.61 & 7.71     &0.185 &0.030 &0.055       &84.67  &86.56 &88.51                                    \\

&{\sc p-fuzz}        &45.62& 63.64& 80.65         &2.77& 7.21& 6.09     &0.049 &0.034 &0.041       &85.73& 88.26& 91.52 \\

&{\sc afl-edge}       &48.25& 48.63& 42.94                    &4.35& 9.99& 11.88       &0.047&0.025&${3.60*e^{-4}}$      &87.64& 89.45& 92.76                                    \\



\hline
\multirow{3}{*}{\sc libxml2} &{\sc pafl}   &61.84 &91.51 &82.15     &7.34 &43.72 &7.04      & ${7.26*e^{-4}}$ &0.011 & 0.064      &87.18  &81.68&88.30                                      \\

&{\sc p-fuzz}   &41.02& 48.47& 51.77     &5.05& 11.70& 21.27      &  ${6.72*e^{-4}}$ &0.014 &0.001      &97.90& 89.26& 97.62                                      \\

&{\sc afl-edge}   &68.92& 69.15& 65.62                       &7.54& 7.59& 29.13      & ${1.07*e^{-4}}$ &0.036 &${1.35*e^{-5}}$                  &98.63& 93.26& 98.24              \\


\hline
\multirow{3}{*}{\sc ffmpeg} &{\sc pafl}       &94.45& 90.67& 91.42      &17.91&23.41&4.09     &0.042 &0.009 &0.381           &86.78& 85.23& 87.01            \\

&{\sc p-fuzz}       &41.64& 62.48& 63.40      &22.63&20.11&6.05     &${0.031}$ &0.049 &${0.004}$           &91.17& 90.22& 98.32            \\

&{\sc afl-edge}   &69.74& 73.47& 62.30      &18.27& 11.62 & 3.26      & 0.006 &0.044 &0.001              &89.90& 90.18& 97.26               \\





\hline
\multirow{3}{*}{\textbf{Ave.}} & {\sc pafl} 
 &\textbf{{66.21}} &\textbf{80.77}&\textbf{79.65} &\textbf{6.86} &\textbf{12.13} &\textbf{3.52} &\textbf{--}&\textbf{--}&\textbf{--}  &\textbf{91.36}&\textbf{90.78}&\textbf{93.35}\\

& {\sc p-fuzz}  
 &\textbf{40.17} &\textbf{45.06}&\textbf{49.51} &\textbf{7.68} &\textbf{8.88} &\textbf{8.04} &\textbf{--}&\textbf{--}&\textbf{--}  &\textbf{95.85}&\textbf{94.83}&\textbf{96.85}\\

& {\sc afl-edge}
&\textbf{60.01}&\textbf{60.32}&\textbf{57.13} &\textbf{10.00} &\textbf{10.20}&\textbf{9.49} &\textbf{--}&\textbf{--} &\textbf{--}  &\textbf{95.80} &\textbf{95.23} &\textbf{97.62} \\

\toprule[0.5pt]
\toprule[0.5pt]
\end{tabular}
\end{table*}


==> tab/afl-stat2.tex <==
\begin{table*}[t!]
\scriptsize
\caption{Statistical results of our evaluation with \afl in 24 hours. In the table, ``\textsf{overlap reduction rate}'' means the average percentage of seeds that the corresponding solution cuts from each instance; ``\textsf{edge coverage increase}'' stands for the increase of code coverage that the corresponding solution brings to \afl; \textsf{p-value} demonstrates the statistical significance of the increase of code coverage (the smaller, the better); and ``\textsf{coverage overlap rate}'' shows how much of the code covered by \afl is also covered by the corresponding solution.}
\label{tab:afl:stat}
\vspace{0.5em}
\begin{tabular}{p{1.5cm}|wl{1.7cm}||p{1.3cm}p{1.3cm}p{1.3cm}|p{1.3cm}p{1.3cm}p{1.3cm}}
\toprule[0.5pt]
\toprule[0.5pt]
\multirow{2} {*}{\textbf{\normalsize{Prog.}}} & 
\multirow{2} {*}{\textbf{\normalsize{Setting}}} &
\multicolumn{6}{c}{\textbf{Statistical evaluation results with 2, 4, and 8 instances.}} \\ 
\cline{3-8} & & \multicolumn{3}{c|}{\textsf{overlap reduction rate}} & \multicolumn{3}{c}{\textsf{edge coverage increase}} \\

\hline
\multirow{3}{*}{\sc objdump} &{\sc pafl}  &60.55\% & 80.77\% & 89.49\%            &1.93\% &0.01\%  & 0.30\%                 
\\
& {\sc p-fuzz}  &46.72\% &53.47\% &62.54\%            &5.08\% & 2.26\% & 3.02\%                 \\

& {\sc afl-edge} & 63.74\% & 63.20\% & 62.37\%             &7.63\% & 7.31\% & 3.06\%         \\




\hline

\multirow{3}{*}{\sc readelf} &{\sc pafl}        &81.23\% &86.81\% &88.41\%          &5.56\% &-3.24\% &-3.58\%                                             \\

&{\sc p-fuzz}        &46.75\% & 43.75\% & 45.37\%          &7.17\% &3.77\% &6.01\%                                           \\

&{\sc afl-edge}  &45.92\% & 43.75\% & 42.47\%          &12.15\% &6.96\% &8.43\%                                          \\


\hline

\multirow{3}{*}{\sc tiff2pdf} &{\sc pafl}  &64.07\% &79.72\% &81.24\%           &3.44\% &0.38\% &4.95\%                                               \\

&{\sc p-fuzz}       &42.18\% & 60.12\% & 64.13\%          &5.50\% &6.27\% &8.48\%                                             \\

&{\sc afl-edge}    &62.38\%& 59.47\%& 58.54\%          &9.01\%& 5.63\%& 11.19\%                  \\




\hline
\multirow{3}{*}{\sc nm-new} &{\sc pafl}    &46.18\% &52.56\% &55.90\%                         &4.04\% &4.76\%  &0.20\%                                             \\

&{\sc p-fuzz}    &43.62\%& 55.63\%& 60.21\%                        &4.52\%& 7.08\%& 3.81\%                                            \\

 &{\sc afl-edge}      &59.87\%& 58.46\%& 60.12\%                        &6.78\%  &6.61\% &3.59\%               \\

\hline

\multirow{3}{*}{\sc nasm} &{\sc pafl}        &64.17\% &82.65\%  &54.70\%          &5.51\% &14.58\%  &2.37\%                                 \\

&{\sc p-fuzz}        &10.01\%& 10.95\%& 8.21\%        &8.93\%& 9.18\%& 8.05\%                            \\

&{\sc afl-edge}    &67.88\%& 68.25\%& 66.84\%                        &13.85\%& 22.59\%& 7.61\%                  \\



\hline

\multirow{3}{*}{\sc tiff2ps} &{\sc pafl}  &57.08\% & 81.93\% & 89.21\%       &7.81\%  &14.99\%  &8.66\%    \\

&{\sc p-fuzz}  &44.00\%& 60.69\%& 66.42\%       &7.50\% & 12.32\% & 9.54\%    \\

&{\sc afl-edge}  &53.36\% &58.46\%  &52.82\%  &10.43\%& 13.52\% & 7.29\%                 \\


\hline
\multirow{3}{*}{\sc tcpdump} &{\sc pafl}        &66.36\% &80.32\% &84.37\%        & 8.20\% &10.61\% & 7.71\%                                      \\

&{\sc p-fuzz}        &45.62\%& 63.64\%& 80.65\%         &2.77\%& 7.21\%& 6.09\%      \\

&{\sc afl-edge}       &48.25\%& 48.63\%& 42.94\%                    &4.35\%& 9.99\%& 11.88\%           \\



\hline
\multirow{3}{*}{\sc libxml2} &{\sc pafl}   &61.84\% &91.51\% &82.15\%     &7.34\% &43.72\% &7.04\%                                          \\

&{\sc p-fuzz}   &41.02\%& 48.47\%& 51.77\%     &5.05\%& 11.70\%& 21.27\%                                           \\

&{\sc afl-edge}   &68.92\%& 69.15\%& 65.62\%                       &7.54\%& 7.59\%& 29.13\%              \\


\hline
\multirow{3}{*}{\sc ffmpeg} &{\sc pafl}       &94.45\%& 90.67\%& 91.42\%      &17.91\%&23.41\%&4.09\%               \\

&{\sc p-fuzz}       &41.64\%& 62.48\%& 63.40\%      &22.63\%&20.11\%&6.05\%          \\

&{\sc afl-edge}   &69.74\%& 73.47\%& 62.30\%      &18.27\%& 11.62\% & 3.26\%          \\





\hline
\multirow{3}{*}{\textbf{Ave.}} & {\sc pafl} 
 &\textbf{{66.21\%}} &\textbf{80.77\%}&\textbf{79.65\%} &\textbf{6.86\%} &\textbf{12.13\%} &\textbf{3.52\%} \\

& {\sc p-fuzz}  
 &\textbf{40.17\%} &\textbf{45.06\%}&\textbf{49.51\%} &\textbf{7.68\%} &\textbf{8.88\%} &\textbf{8.04\%} \\

& {\sc afl-edge}
&\textbf{60.01\%}&\textbf{60.32\%}&\textbf{57.13\%} &\textbf{10.00\%} &\textbf{10.20\%}&\textbf{9.49\%}  \\

\toprule[0.5pt]
\toprule[0.5pt]
\end{tabular}
\vspace{-1em}
\end{table*}



\addtocounter{table}{-1}



\begin{table*}[t!]
\scriptsize
\captionsetup{list=no}
\caption{ (continued)}
\label{tab:afl:stat}
\vspace{0.5em}
\begin{tabular}{p{1.5cm}|wl{1.7cm}||p{1.3cm}p{1.3cm}p{1.3cm}|p{1.3cm}p{1.3cm}p{1.3cm}}
\toprule[0.5pt]
\toprule[0.5pt]
\multirow{2} {*}{\textbf{\normalsize{Prog.}}} & 
\multirow{2} {*}{\textbf{\normalsize{Setting}}} &
\multicolumn{6}{c}{\textbf{Statistical evaluation results with 2, 4, and 8 instances.}} \\ 
\cline{3-8} & & \multicolumn{3}{c|}{\textsf{p-value}} & \multicolumn{3}{c}{\textsf{coverage overlap rate}} \\

\hline
\multirow{3}{*}{\sc objdump} 
&{\sc pafl}    &0.321    &0.715    &0.102      &95.46\% &94.87\% &95.81\%               \\
& {\sc p-fuzz}  & 0.072   & 0.032   & ${2.91*e^{-4}}$      &96.82\% &96.27\% &97.89\%  \\
& {\sc afl-edge}  & 0.001 & 0.038 & 0.025                       &97.54\% & 98.34\% & 98.53\% \\




\hline

\multirow{3}{*}{\sc readelf} 
&{\sc pafl}    &0.033  &0.189  &0.117      & 92.54\% &92.13\% &92.87\%    \\

&{\sc p-fuzz}    &0.040  &0.006  &${3.92*e^{-5}}$                &98.85\% &98.51\% &97.96\%     \\

&{\sc afl-edge}  &0.050  &0.020  & 0.001       &97.52\% &97.21\% &97.69\%   \\


\hline

\multirow{3}{*}{\sc tiff2pdf} 
&{\sc pafl}  &0.004 &0.049 &0.293      &96.96\% &91.28\% &93.81\%  \\

&{\sc p-fuzz}     &0.007 &0.040 &0.042               &98.51\% &97.06\% &97.91\%    \\

&{\sc afl-edge}    &${7.69*e^{-5}}$&0.021&${2.96*e^{-4}}$       &98.49\%& 95.98\%& 99.14\%   \\




\hline
\multirow{3}{*}{\sc nm-new} 
&{\sc pafl}        &0.098  &0.072  & 0.187                &96.64\% &96.18\%  &97.53\%     \\

&{\sc p-fuzz}      & 0.001 &0.032 &0.002               &97.63\%& 98.14\%& 98.12\%     \\

 &{\sc afl-edge}    &0.027 &0.076 &0.001               &96.25\%& 96.85\%& 98.53\%     \\

\hline

\multirow{3}{*}{\sc nasm} 
&{\sc pafl}       &0.050   &0.012  &0.057               &99.78\% &99.25\%  &99.78\%        \\

&{\sc p-fuzz}     & ${2.46*e^{-6}}$ &${2.32*e^{-5}}$ &${3.64*e^{-6}}$              &98.96\%& 98.33\%& 94.25\%  \\

&{\sc afl-edge}    & ${1.73*e^{-8}}$ & ${1.85*e^{-7}}$ &${1.43*e^{-4}}$              &99.24\%& 99.26\%& 99.26\%    \\



\hline

\multirow{3}{*}{\sc tiff2ps} 
&{\sc pafl}   &0.034 & 0.019 &0.024  &82.25\% & 89.85\%& 96.56\%     \\

&{\sc p-fuzz}  &${8.24*e^{-4}}$&${5.74*e^{-8}}$&${6.63*e^{-4}}$  &97.05\% & 97.45\% & 98.02\%   \\

&{\sc afl-edge}  & ${1.66*e^{-5}}$ &${5.01*e^{-5}}$ &${5.88*e^{-4}}$    & 96.98\% & 96.50\%& 97.15\%  \\


\hline
\multirow{3}{*}{\sc tcpdump} 
&{\sc pafl}     &0.185 &0.030 &0.055       &84.67\%  &86.56\% &88.51\%      \\

&{\sc p-fuzz}     &0.049 &0.034 &0.041       &85.73\%& 88.26\%& 91.52\%       \\

&{\sc afl-edge}     &0.047&0.025&${3.60*e^{-4}}$      &87.64\%& 89.45\%& 92.76\%       \\



\hline
\multirow{3}{*}{\sc libxml2} 
&{\sc pafl}    & ${7.26*e^{-4}}$ &0.011 & 0.064      &87.18\%  &81.68\%&88.30\%   \\

&{\sc p-fuzz}      &  ${6.72*e^{-4}}$ &0.014 &0.001      &97.90\%& 89.26\%& 97.62\%      \\

&{\sc afl-edge}   & ${1.07*e^{-4}}$ &0.036 &${1.35*e^{-5}}$                  &98.63\%& 93.26\%& 98.24\% \\


\hline
\multirow{3}{*}{\sc ffmpeg} 
&{\sc pafl}       &0.042 &0.009 &0.381           &86.78\%& 85.23\%& 87.01\%          \\

&{\sc p-fuzz}       &${0.031}$ &0.049 &${0.004}$           &91.17\%& 90.22\%& 98.32\%      \\

&{\sc afl-edge}    & 0.006 &0.044 &0.001              &89.90\%& 90.18\%& 97.26\%   \\





\hline
\multirow{3}{*}{\textbf{Ave.}} 
 & {\sc pafl}  &\textbf{--}&\textbf{--}&\textbf{--}  &\textbf{91.36\%}&\textbf{90.78\%}&\textbf{93.35\%}
 \\

& {\sc p-fuzz}  &\textbf{--}&\textbf{--}&\textbf{--} &\textbf{95.85\%}&\textbf{94.83\%}&\textbf{96.85\%}
  \\

& {\sc afl-edge} &\textbf{--}&\textbf{--} &\textbf{--}  &\textbf{95.80\%} &\textbf{95.23\%} &\textbf{97.62\%} \\

\toprule[0.5pt]
\toprule[0.5pt]
\end{tabular}
\vspace{-1em}
\end{table*}




==> tab/code-cov.tex <==
% \begin{table*}[t!]
\renewcommand{\arraystretch}{0.3}
\centering
% \begin{adjustwidth}{-0.15cm}{}
 \begin{longtable}{wc{4.5cm}wc{4.5cm}wc{4.5cm}}
         \includegraphics[scale=0.075]{eval_result/objdump_2_instance_afl.pdf} & 
         \includegraphics[scale=0.075]{eval_result/objdump_4_instance_afl.pdf} &
         \includegraphics[scale=0.075]{eval_result/objdump_8_instance_afl.pdf} 
        % \includegraphics[scale=0.054]{eval_result/objdump_2_instance_qsym.pdf} &
        %  \includegraphics[scale=0.054]{eval_result/objdump_4_instance_qsym.pdf} & 
        % \includegraphics[scale=0.054]{eval_result/objdump_8_instance_qsym.pdf} 
         \\
         {\scriptsize\textbf{objdump} \scriptsize 2 instances AFL} &
         {\scriptsize\textbf{objdump} \scriptsize 4 instances AFL} &
         {\scriptsize\textbf{objdump} \scriptsize 8 instances AFL} 
        %  {\scriptsize\textbf{objdump} \scriptsize 2 instance QSYM} &
        %  {\scriptsize\textbf{objdump} \scriptsize 4 instance QSYM} &
        %  {\scriptsize\textbf{objdump} \scriptsize 8 instance QSYM} \\
         \\
         
         \includegraphics[scale=0.075]{eval_result/readelf_2_instance_afl.pdf} & 
         \includegraphics[scale=0.075]{eval_result/readelf_4_instance_afl.pdf} &
         \includegraphics[scale=0.075]{eval_result/readelf_8_instance_afl.pdf} 
        %  \includegraphics[scale=0.054]{eval_result/readelf_2_instance_qsym.pdf} &
        %  \includegraphics[scale=0.054]{eval_result/readelf_4_instance_qsym.pdf} & 
        % \includegraphics[scale=0.054]{eval_result/readelf_8_instance_qsym.pdf} 
         \\
         {\scriptsize\textbf{readelf} \scriptsize 2 instances AFL} &
         {\scriptsize\textbf{readelf} \scriptsize 4 instances AFL} &
         {\scriptsize\textbf{readelf} \scriptsize 8 instances AFL} 
        %  {\scriptsize\textbf{readelf} \scriptsize 2 instance QSYM} &
        %  {\scriptsize\textbf{readelf} \scriptsize 4 instance QSYM} &
        %  {\scriptsize\textbf{readelf} \scriptsize 8 instance QSYM} \\
         \\
         \includegraphics[scale=0.075]{eval_result/tiff2pdf_2_instance_afl.pdf} & 
         \includegraphics[scale=0.075]{eval_result/tiff2pdf_4_instance_afl.pdf} &
         \includegraphics[scale=0.075]{eval_result/tiff2pdf_8_instance_afl.pdf} 
        %  \includegraphics[scale=0.054]{eval_result/tiff2pdf_2_instance_qsym.pdf} &
        %  \includegraphics[scale=0.054]{eval_result/tiff2pdf_4_instance_qsym.pdf} & 
        % \includegraphics[scale=0.054]{eval_result/tiff2pdf_8_instance_qsym.pdf} 
         \\
         {\scriptsize\textbf{tiff2pdf} \scriptsize 2 instances AFL} &
         {\scriptsize\textbf{tiff2pdf} \scriptsize 4 instances AFL} &
         {\scriptsize\textbf{tiff2pdf} \scriptsize 8 instances AFL} 
        %  {\scriptsize\textbf{tiff2pdf} \scriptsize 2 instance QSYM} &
        %  {\scriptsize\textbf{tiff2pdf} \scriptsize 4 instance QSYM} &
        %  {\scriptsize\textbf{tiff2pdf} \scriptsize 8 instance QSYM} \\
         \\
         \includegraphics[scale=0.075]{eval_result/nm_2_instance_afl.pdf} & 
         \includegraphics[scale=0.075]{eval_result/nm_4_instance_afl.pdf} &
         \includegraphics[scale=0.075]{eval_result/nm_8_instance_afl.pdf} 
        %  \includegraphics[scale=0.054]{eval_result/nm_2_instance_qsym.pdf} &
        %  \includegraphics[scale=0.054]{eval_result/nm_4_instance_qsym.pdf} & 
        % \includegraphics[scale=0.054]{eval_result/nm_8_instance_qsym.pdf} 
         \\
         {\scriptsize\textbf{nm-new} \scriptsize 2 instances AFL} &
         {\scriptsize\textbf{nm-new} \scriptsize 4 instances AFL} &
         {\scriptsize\textbf{nm-new} \scriptsize 8 instances AFL} 
        %  {\scriptsize\textbf{nm-new} \scriptsize 2 instance QSYM} &
        %  {\scriptsize\textbf{nm-new} \scriptsize 4 instance QSYM} &
        %  {\scriptsize\textbf{nm-new} \scriptsize 8 instance QSYM} \\
         \\
         \includegraphics[scale=0.075]{eval_result/nasm_2_instance_afl.pdf} & 
         \includegraphics[scale=0.075]{eval_result/nasm_4_instance_afl2.pdf} &
         \includegraphics[scale=0.075]{eval_result/nasm_8_instance_afl.pdf}  
        % \includegraphics[scale=0.054]{eval_result/nasm_2_instance_qsym.pdf} &
        %  \includegraphics[scale=0.054]{eval_result/nasm_4_instance_qsym2.pdf} & 
        % \includegraphics[scale=0.054]{eval_result/nasm_8_instance_qsym.pdf}
         \\
         {\scriptsize\textbf{nasm} \scriptsize 2 instances AFL} &
         {\scriptsize\textbf{nasm} \scriptsize 4 instances AFL} &
         {\scriptsize\textbf{nasm} \scriptsize 8 instances AFL} 
        %  {\scriptsize\textbf{nasm} \scriptsize 2 instance QSYM} &
        %  {\scriptsize\textbf{nasm} \scriptsize 4 instance QSYM} &
        %  {\scriptsize\textbf{nasm} \scriptsize 8 instance QSYM} \\
         \\
         \includegraphics[scale=0.075]{eval_result/tiff2ps_2_instance_afl.pdf} & 
         \includegraphics[scale=0.075]{eval_result/tiff2ps_4_instance_afl.pdf} &
         \includegraphics[scale=0.075]{eval_result/tiff2ps_8_instance_afl.pdf} 
        %  \includegraphics[scale=0.054]{eval_result/tiff2ps_2_instance_qsym.pdf} &
        %  \includegraphics[scale=0.054]{eval_result/tiff2ps_4_instance_qsym.pdf} &
        %  \includegraphics[scale=0.054]{eval_result/tiff2ps_8_instance_qsym.pdf} \\
         
         \\
         {\scriptsize\textbf{tiff2ps} \scriptsize 2 instances AFL} &
         {\scriptsize\textbf{tiff2ps} \scriptsize 4 instances AFL} &
         {\scriptsize\textbf{tiff2ps} \scriptsize 8 instances AFL} 
        %  {\scriptsize\textbf{tiff2ps} \scriptsize 2 instance QSYM} &
        %  {\scriptsize\textbf{tiff2ps} \scriptsize 4 instance QSYM} &
        %  {\scriptsize\textbf{tiff2ps} \scriptsize 8 instance QSYM} \\
         \\
         
         \includegraphics[scale=0.075]{eval_result/tcpdump_2_instance_afl.pdf} & 
         \includegraphics[scale=0.075]{eval_result/tcpdump_4_instance_afl.pdf} &
         \includegraphics[scale=0.075]{eval_result/tcpdump_8_instance_afl.pdf}  
        % \includegraphics[scale=0.054]{eval_result/tcpdump_2_instance_qsym.pdf} &
        %  \includegraphics[scale=0.054]{eval_result/tcpdump_4_instance_qsym.pdf} & 
        %\includegraphics[scale=0.054]{eval_result/tcpdump_8_instance_qsym.pdf} 
         \\
         {\scriptsize\textbf{tcpdump} \scriptsize 2 instances AFL} &
         {\scriptsize\textbf{tcpdump} \scriptsize 4 instances AFL} &
         {\scriptsize\textbf{tcpdump} \scriptsize 8 instances AFL} 
        %  {\scriptsize\textbf{tcpdump} \scriptsize 2 instance QSYM} &
        %  {\scriptsize\textbf{tcpdump} \scriptsize 4 instance QSYM} &
        %  {\scriptsize\textbf{tcpdump} \scriptsize 8 instance QSYM} \\
         \\
         \includegraphics[scale=0.075]{eval_result/libxml_2_instance_afl.pdf} & 
         \includegraphics[scale=0.075]{eval_result/libxml_4_instance_afl.pdf} &
         \includegraphics[scale=0.075]{eval_result/libxml_8_instance_afl.pdf} 
         %\includegraphics[scale=0.054]{eval_result/libxml_2_instance_qsym.pdf} &
        %  \includegraphics[scale=0.054]{eval_result/libxml_4_instance_qsym.pdf} & 
        %\includegraphics[scale=0.054]{eval_result/libxml_8_instance_qsym.pdf} 
         \\
         {\scriptsize\textbf{libxml} \scriptsize 2 instances AFL} &
         {\scriptsize\textbf{libxml} \scriptsize 4 instances AFL} &
         {\scriptsize\textbf{libxml} \scriptsize 8 instances AFL}
        %  {\scriptsize\textbf{libxml} \scriptsize 2 instance QSYM} &
        %  {\scriptsize\textbf{libxml} \scriptsize 4 instance QSYM} &
        %  {\scriptsize\textbf{libxml} \scriptsize 8 instance QSYM} \\
         \\
         \includegraphics[scale=0.075]{eval_result/ffmpeg_2_instance_afl.pdf} & 
         \includegraphics[scale=0.075]{eval_result/ffmpeg_4_instance_afl.pdf} &
         \includegraphics[scale=0.075]{eval_result/ffmpeg_8_instance_afl.pdf} 
         %\includegraphics[scale=0.054]{eval_result/ffmpeg_2_instance_qsym.pdf} &
        %  \includegraphics[scale=0.054]{eval_result/ffmpeg_4_instance_qsym.pdf} & 
        %\includegraphics[scale=0.054]{eval_result/ffmpeg_8_instance_qsym.pdf} 
         \\
         
         {\scriptsize\textbf{ffmpeg} \scriptsize 2 instances AFL} &
         {\scriptsize\textbf{ffmpeg} \scriptsize 4 instances AFL} &
         {\scriptsize\textbf{ffmpeg} \scriptsize 8 instances AFL}
        %  {\scriptsize\textbf{ffmpeg} \scriptsize 2 instance QSYM} &
        %  {\scriptsize\textbf{ffmpeg} \scriptsize 4 instance QSYM} &
        %  {\scriptsize\textbf{ffmpeg} \scriptsize 8 instance QSYM} 
         
\end{longtable}
\vspace{0.5em}
% \end{adjustwidth}
\captionof{figure}{Results of code coverage with our 9 benchmark programs across 24 hours. }
% The \emph{left} part shows the results of \afl and the \emph{right} part shows the results of \qsym.}

% \captionof{figure}{Results of code coverage with our 9 benchmark programs across 24 hours. The \emph{left} part shows the results of \afl and the \emph{right} part shows the results of \qsym. In the legends, {\tt without\_split} stands for stock \afl/\qsym; {\tt with\_path\_split} means \afl/\qsym with our path-coverage-based task distribution; and {\tt with\_edge\_split} represents \afl/\qsym with our edge-coverage-based task distribution.}
\label{fig:codecov}
% \end{table*}


==> tab/multi-mut.tex <==
\begin{table}[t!]
\scriptsize
\centering
\caption{Results of multiple mutation rounds. {\tt Cov} indicates the code coverage after current mutation round. {\tt Rate} represents the code coverage increasing rate after mutation.}
\label{tab:multi-mut:increase}
\begin{tabular}{p{1.2cm}|p{0.4cm}p{0.4cm}|p{0.4cm}p{0.6cm}|p{0.4cm}p{0.6cm}|p{0.4cm}p{0.6cm}}
\toprule[0.5pt]
\toprule[0.5pt]
%%%
%%%
\multirow{3}{*}{\bf{\normalsize{\em Program}}}  & \multicolumn{8}{c}{\bf{\normalsize{\em Mut. Rounds \& Cov. Increase Rate }}} \\\cline{2-9}
 & \multicolumn{2}{c|}{Round 1}
 & \multicolumn{2}{c|}{Round 2}
 & \multicolumn{2}{c|}{Round 3}
 & \multicolumn{2}{c}{Round 4}\\
 \cline{2-9}
 & {\tt Cov}
 & Rate
& {\tt Cov}
 & Rate
 & {\tt Cov}
 & Rate
  & {\tt Cov}
 & Rate\\\hline
{\sc Objdump} & 18778 & - & 19103 & 1.731\% & 19331 & 1.193\% & 19454 & 0.636\%  \\
\rowcolor{mygray}
{\sc Tiff2ps} & 16122 & - & 16341 & 1.358\% & 16391 & 0.306\% & 16407 & 0.097\%  \\
{\sc Libxml} & 27282 & - & 27350 & 0.229\% & 27379 & 0.106\% & 27384 & 0.018\%  \\
\rowcolor{mygray}
{\sc Nm-new} & 6619 & - & 6706 & 1.314\% & 6742 & 0.573\% & 6761 & 0.282\%  \\

\hline

{\bf Ave. } & {\bf 17200} & - & {\bf 17375} & {\bf 1.02\%} & {\bf 17460} & {\bf 0.489\%} & {\bf 17501} & {\bf 0.234\%}  \\

 %\rowcolor{mygray} 
\bottomrule[0.5pt]
\bottomrule[0.5pt]
\end{tabular}
\end{table}

==> tab/qsym-stat.tex <==
\begin{table*}[t!]
\scriptsize
\caption{Statistical results of our evaluation with \qsym in 24 hours. Organization of columns follows Table~\ref{tab:afl:stat}.}
\label{tab:qsym:stat}
\vspace{0.5em}
\begin{tabular}{p{0.85cm}|wl{1.0cm}||p{0.70cm}p{0.70cm}p{0.80cm}|p{0.74cm}p{0.74cm}p{0.74cm}|p{1.1cm}p{1.1cm}p{1.2cm}|p{0.85cm}p{0.85cm}p{0.70cm}}
\toprule[0.5pt]
\toprule[0.5pt]
\multirow{2}{*}{\textbf{\normalsize{Prog.}}} & 
\multirow{2}{*}{\textbf{\normalsize{Setting}}} &
\multicolumn{12}{c}{\textbf{\large{Statistical evaluation results with 2, 4, and 8 instances (\qsym).}}} \\ \cline{3-14}
&& \multicolumn{3}{c|}{\textsf{overlap reduction rate}} & \multicolumn{3}{c|}{\textsf{edge coverage increase}} & \multicolumn{3}{c|}{\textsf{p-value}} & \multicolumn{3}{c}{\textsf{coverage overlap rate}} \\\hline


\multirow{3}{*}{\sc objdump} &{\sc pafl} &62.21\% &61.11\% &67.24\%            &1.01\% &8.36\% &7.00\%                &0.860 &0.146 & 0.166      &92.55\% &82.95\% &86.51\%                                    \\


&{\sc p-fuzz} &40.79\% &55.94\% &62.93\%            &10.00\% & 7.28\% &10.34\%                & 0.004   & 0.038   & ${1.70*e^{-5}}$      &95.45\% &92.81\%& 92.44\%                                    \\

&{\sc afl-edge} & 61.73\% & 62.75\% & 61.86\%             &1.57\% & 6.42\% & 13.24\%         & 0.031 & 0.007  &${1.62*e^{-4}}$                        &93.27\% & 83.68\% & 97.54\% \\




\hline
\multirow{3}{*}{\sc readelf} &{\sc pafl}        &79.25\% &91.10\% &88.11\%          &8.42\%&2.15\% &8.36\%        &0.067  &0.372  &0.136                &92.56\% &91.62\% &88.29\%                                     \\


&{\sc p-fuzz}        &46.94\% & 66.51\% & 74.78\%          &2.85\%& 8.89\%& 5.95\%        &0.084  &${3.47*e^{-4}}$  &0.172                &98.07\%& 98.11\%& 92.36\%                                     \\

&{\sc afl-edge}  &42.58\% & 45.34\% & 49.91\%          &9.78\%& 6.48\%& 9.01\%        &0.055  &0.024  & 0.024       &98.17\%& 97.86\%& 98.85\%                                     \\

\hline
\multirow{3}{*}{\sc tiff2pdf} &{\sc pafl}       &62.40\% &83.99\% &92.20\%          &2.63\%&13.19\%&-2.20\%          &0.067 &0.004 &0.159               &95.82\% &91.68\% &93.22\%                                     \\

&{\sc p-fuzz}       &42.67\% & 58.04\%& 15.56\%          &2.23\%& 8.76\%& 7.77\%          &0.046 &0.016 &${8.76*e^{-4}}$               &96.26\%& 98.47\%& 94.26\%                                     \\

&{\sc afl-edge}    &60.69\%& 58.58\%& 57.18\%          &3.46\%& 3.10\%& 6.78\%         &0.063 &0.032 &0.007       &96.98\%& 97.69\%& 97.69\%                                     \\


\hline
\multirow{3}{*}{\sc nm-new} &{\sc pafl}    &63.56\% &78.99\% & 86.67\%                        &3.96\% &-4.17\% 
&5.36\%           &0.162  &0.552 &0.199               &86.85\% &82.13\% &92.17\%                        \\

&{\sc p-fuzz}    &12.03\%& 13.84\%& 11.32\%                        &14.82\%& 25.46\%& 11.80\%           & ${1.73*e^{-4}}$ &0.060 &${3.73*e^{-4}}$               &97.33\%&82.85\%&98.01\%                        \\

&{\sc afl-edge}               &56.53\%& 56.83\%& 57.29\%                        &25.02\%& 26.26\%& 49.13\%         &0.001 &0.002 &${9.61*e^{-8}}$               &97.46\%& 83.27\%& 93.33\%        \\

\hline
\multirow{3}{*}{\sc nasm} &{\sc pafl}         &61.11\% &83.80\% &83.25\%            &2.19\% &-0.18\% &4.31\%            &0.120 &0.826 &0.135              &97.93\% &91.87\% &94.22\%              \\

&{\sc p-fuzz}         &12.03\% & 13.84\% & 10.57\%            &6.54\% &3.85\% &11.80\%            &${1.73*e^{-4}}$ &0.060 & ${3.73*e^{-4}}$             &98.45\% &97.19\% &99.07\%              \\

&{\sc afl-edge}     &66.65\%& 65.27\%& 67.22\%          &6.46\%& 13.17\%& 8.13\%     &0.070 &0.041 &0.044     &98.05\% & 95.75\% & 98.96\%                                     \\

\hline
\multirow{3}{*}{\sc tiff2ps} &{\sc pafl}  &75.27\% &80.62\% & 87.38\%                      &6.73\% &5.13\% &2.82\%          &0.047 &0.051 & 0.038              &96.91\% &91.25\% &88.05\%       \\

&{\sc p-fuzz}  &44.30\%& 59.94\%& 69.99\%                      &13.19\%& 6.70\%& 2.82\%          &0.002 &0.008 &0.019               &97.24\%& 94.98\%& 97.07\%       \\

&{\sc afl-edge}    &60.51\%& 56.07\%& 50.98\%                        &15.60\%& 20.38\%& 7.78\%           & ${1.55*e^{-7}}$ &${3.30*e^{-7}}$ &0.008               &98.29\%& 96.89\%& 97.83\%                   \\

\hline
\multirow{3}{*}{\sc tcpdump} &{\sc pafl}  &67.57\% &84.31\% &80.66\%                      &7.56\% &3.95\%&0.36\%          &0.039 &0.046 &0.018               &87.17\% &80.93\% &83.73\%       \\

&{\sc p-fuzz}  &46.40\%& 67.72\%& 77.54\%                      &2.44\%& 2.25\%& 0.84\%          &0.049 &0.050 &0.004               &87.19\%& 88.38\%& 87.00\%       \\

&{\sc afl-edge}  &54.57\%& 53.04\%& 43.94\%                      &4.45\%& 4.78\%& 8.65\%          &0.047 &0.047 &0.007               &88.48\%& 89.13\%& 90.46\%       \\


\hline

\multirow{3}{*}{\sc libxml2} &{\sc pafl}    &59.34\% &74.82\% &83.32\%                       &27.21\%&33.59\% &136.52\%       &${1.01*e^{-4}}$ &0.027 &${1.21*e^{-8}}$                        &97.45\% &85.29\% &89.80\%     \\
&{\sc p-fuzz}    &6.68\%& 6.11\%& 3.37\%                       &16.09\%& 41.83\%& 37.87\%       &${2.24*e^{-4}}$ &0.042 &0.005                        &99.51\%& 89.51\%& 98.85\%     \\
&{\sc afl-edge}   &70.77\%& 71.46\%& 67.85\%                       &13.77\%& 39.31\%&56.40\%             &${1.44*e^{-4}}$ &0.021 &0.001                  &99.37\%& 90.16\%& 98.27\%      \\

\hline

\multirow{3}{*}{\sc ffmpeg} &{\sc pafl}    &50.91\% &72.78\% &89.78\%     &22.81\%&9.28\%&11.72\%            &0.038 &0.035 &0.056             &80.81\% &88.39\% &85.58\%        \\

&{\sc p-fuzz}    &38.89\%& 59.14\%& 71.34\%     &12.37\%& 6.05\%& 18.92\%            &0.046 &0.040 &0.045             &91.37\%& 95.02\%& 96.59\%        \\

&{\sc afl-edge}   &64.33\%& 56.92\%& 23.24\%                      &26.37\%& 11.87\%& 29.67\%          &0.013 &0.010 &0.005                  &90.02\%& 93.77\%& 97.66\%        \\

\hline
\multirow{3}{*}{\textbf{Ave.}} & {\sc pafl}  
 &\textbf{64.63\%} &\textbf{79.06\%}&\textbf{84.29\%} &\textbf{9.17\%} &\textbf{7.92\%} &\textbf{19.36\%} &\textbf{--}&\textbf{--}&\textbf{--}  &\textbf{91.95\%}&\textbf{87.34\%}&\textbf{89.06\%}
\\


& {\sc p-fuzz}  
 &\textbf{31.80\%} &\textbf{43.81\%}&\textbf{48.93\%} &\textbf{8.95\%} &\textbf{12.34\%} &\textbf{12.01\%} &\textbf{--}&\textbf{--}&\textbf{--}  &\textbf{95.65\%}&\textbf{93.04\%}&\textbf{95.07\%}
\\

& {\sc afl-edge}  
&\textbf{59.82\%}&\textbf{58.47\%}&\textbf{59.63\%} &\textbf{11.83\%} &\textbf{14.64\%}&\textbf{20.98\%} &\textbf{--}&\textbf{--} &\textbf{--}  &\textbf{95.57\%} &\textbf{92.02\%} &\textbf{96.73\%} \\

\toprule[0.5pt]
\toprule[0.5pt]
\end{tabular}
\end{table*}

